miniCTX: Neural Theorem Proving with (Long-)Contexts

Real-world formal theorem proving often depends on a wealth of context, including definitions, lemmas, comments, file structure, and other information. We introduce miniCTX, which tests a model's ability to prove formal mathematical theorems that depend on new context that is not seen during training. miniCTX contains theorems sourced from real Lean projects and textbooks, each associated with a context that can span tens of thousands of tokens. Models are tasked with proving a theorem given access to code from the theorem's repository, which contains context that is needed for the proof. As a baseline for miniCTX, we tested fine-tuning and prompting methods that condition theorem proving on preceding context. Both approaches substantially outperform traditional methods that rely solely on state information. We found that this ability to use context is not captured by previous benchmarks such as miniF2F. Alongside miniCTX, we offer ntp-toolkit for automatically extracting and annotating theorem proving data, making it easy to add new projects into miniCTX to ensure that contexts are not seen during training. miniCTX offers a challenging and realistic evaluation of neural theorem provers.

==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,  % thomas: changed to true to avoid very weird error

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

% (Thomas) added: treat ` as ` and not back single quote
upquote=true,
}

==> sections/97-datasheet.tex <==
\section{Datasheet}
We present a datasheet~\citep{gebru2021datasheets} for \dsname.

\subsection{Motivation}
\paragraph{For what purpose was the dataset created?}
The dataset was created to evaluate the ability of models to prove formal mathematical theorems that depend on new definitions, lemmas, or other contextual information not observed during training. It is designed to provide a challenging and realistic scenario.
\paragraph{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organisation)?}
The dataset was created by Jiewen Hu, Thomas Zhu, and Sean Welleck from the L3 lab at Carnegie Mellon University.
\paragraph{Who funded the creation of the dataset?}
L3 lab.

\subsection{Composition}
\paragraph{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}
Each instance represents a mathematical theorem stated in Lean, including both theorem statements and corresponding preceding file context, as well as other related metadata for further analysis. See \S\ref{sec:example-entry} for an example.
\paragraph{How many instances are there in total (of each type, if appropriate)?}
The dataset contains 201 samples in total from four different projects: PrimeNumberTheoremAnd with 47 problems, PFR with 54 problems, Math2001 with 50 problems, and Mathlib with 50 problems.
\paragraph{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}
\dsname\ is a sample of 201 theorems from some recent projects. It is not exhaustive of all possible instances, but rather a curated selection meant to provide a comprehensive and challenging scenario for testing theorem proving. We also offer automated tools and guidelines to extract more instances from any Lean project.
\paragraph{What data does each instance consist of?}
Each theorem instance includes a declaration, context (file content up to the declaration), its proof and other metadata (see~\S \ref{sec:data_example}).
\paragraph{Is there a label or target associated with each instance?}
We include the original proof for each theorem if it exists in the original file; however, the original proof only serves as an example. The accuracy of generated proofs is evaluated by the Lean compiler, and we provide the evaluation code. Note that we train models on an extracted context-state-tactic dataset (see~\S\ref{apx:ssec:data-extraction}) and only use \dsname\ for evaluation.
\paragraph{Is any information missing from individual instances?}
Some instances in the dataset are designed as exercises for readers or as open problems, and consequently, do not have example proofs.
\paragraph{Are relationships between individual instances made explicit (e.g., users' movie ratings, social network links)?}
Yes, we include metadata information about the file from which each theorem is extracted, as well as its relative position in a file and whether it uses other premises.
\paragraph{Are there recommended data splits (e.g., training, development/validation, testing)?}
The dataset has different splits for different source project. In addition, we recommend users to look at metadata for more insteresting splits (for example, the dependency level studied in experiment section).
\paragraph{Are there any errors, sources of noise, or redundancies in the dataset?}
We do not expect any errors that affect evaluation.
\paragraph{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?}
We extract the dataset from recent Lean projects and provide their links and versions. 
\paragraph{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor–patient confidentiality, data that includes the content of individuals’ non-public communications)?}
The dataset only includes publicly available code. We do not publicly release the Math2001 split because of it is under copyright.
\paragraph{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}
No.

\subsection{Collection Process}

\paragraph{How was the data associated with each instance acquired?}
We manually selected and collected theorems for \dsname\ from respective sources, although we note this can be automated with \textsc{NTP-TOOLKIT}.
\paragraph{What mechanisms or procedures were used to collect the data (e.g., hardware apparatuses or sensors, manual human curation, software programs, software APIs)?}
See the previous question.
\paragraph{If the dataset is a sample from a larger set, what was the sampling strategy (e.g., deterministic, probabilistic with specific sampling probabilities)?}
We manually picked a wide range of theorems with different traits and difficulties, specifically we focus on how the theorem proof rely on the context.
\paragraph{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}
The authors collected the data.
\paragraph{Over what timeframe was the data collected?}
The data was collected in April and May 2024.
\paragraph{Were any ethical review processes conducted (e.g., by an institutional review board)?}
No.

\subsection{Preprocessing/Cleaning/Labelling}
\paragraph{Was any preprocessing/cleaning/labelling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?}
We do little preprocessing on the data; see the data format in \S\ref{sec:example-entry}.
\paragraph{Was the ``raw'' data saved in addition to the preprocessed/cleaned/labelled data (e.g., to support unanticipated future uses)?}
\dsname\ was extracted from corresponding GitHub repositories, see miniCTX section for more details.
\paragraph{Is the software that was used to preprocess/clean/label the data available?}
N/A.


\subsection{Uses}

\paragraph{Has the dataset been used for any tasks already?}
We have already employed the \dsname \  dataset to evaluate various fine-tuning and prompting methods that utilize context information in different ways. This evaluation highlights the significant impact of incorporating context in theorem proving tasks.
\paragraph{Is there a repository that links to any or all papers or systems that use the dataset?}
N/A.
\paragraph{What (other) tasks could the dataset be used for?}
None.
\paragraph{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labelled that might impact future uses?}
For future uses we will continue updating the dataset with recent projects so that newer language models have not seen entries in the dataset.
\paragraph{Are there tasks for which the dataset should not be used?}
N/A.

\subsection{Distribution}

\paragraph{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organisation) on behalf of which the dataset was created?}
The dataset is publicly available and can be accessed on Hugging Face: \href{https://huggingface.co/datasets/l3lab/miniCTX}{https://huggingface.co/datasets/l3lab/miniCTX}.

\paragraph{How will the dataset be distributed (e.g., tarball on website, API, GitHub)?}
It is released on HuggingFace.
\paragraph{When will the dataset be distributed?}
It is already released.
\paragraph{Will the dataset be distributed under a copyright or other intellectual property (IP) licence, and/or under applicable terms of use (ToU)?}
We release \dsname\ under the Apache 2.0 license. The dataset is extracted from various repositories, which are under their respective copyrights. \toolkit\ is released under the MIT license.
\paragraph{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}
The usage and redistribution of the data in the miniCTX dataset are subject to the licenses of their original projects. The licenses for the publicly available splits in our dataset are as follows:
\begin{enumerate}
\item PrimeNumberTheoremAnd: Apache-2.0 license
\item PFR: Apache-2.0 license
\item Mathlib: Apache-2.0 license
\end{enumerate}
These licenses permit the use, modification, and redistribution of the dataset under specified conditions, aligning with open-source principles.
\paragraph{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?}
No.



\subsection{Maintenance}

\paragraph{Who will be supporting/hosting/maintaining the dataset?}
The authors, members of L3 lab, will maintain the dataset.
\paragraph{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}
Jiewen Hu: jiewenh@andrew.cmu.edu
\paragraph{Is there an erratum?}
No.
\paragraph{Will the dataset be updated (e.g., to correct labelling errors, add new instances, delete instances)?}
The dataset will be updated to include newer examples.
\paragraph{Will older versions of the dataset continue to be supported/hosted/maintained?}
Yes.
\paragraph{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}
We provide automated extraction tools \textsc{NTP-TOOLKIT}.
\paragraph{Any other comments?}
None.

